All in the Exponential Family: Bregman Duality in Thermodynamic Variational Inference

The recently proposed Thermodynamic Variational Objective (TVO) leverages thermodynamic integration to provide a family of variational inference objectives, which both tighten and generalize the ubiquitous Evidence Lower Bound (ELBO). However, the tightness of TVO bounds was not previously known, an expensive grid search was used to choose a "schedule" of intermediate distributions, and model learning suffered with ostensibly tighter bounds. In this work, we propose an exponential family interpretation of the geometric mixture curve underlying the TVO and various path sampling methods, which allows us to characterize the gap in TVO likelihood bounds as a sum of KL divergences. We propose to choose intermediate distributions using equal spacing in the moment parameters of our exponential family, which matches grid search performance and allows the schedule to adaptively update over the course of training. Finally, we derive a doubly reparameterized gradient estimator which improves model learning and allows the TVO to benefit from more refined bounds. To further contextualize our contributions, we provide a unified framework for understanding thermodynamic integration and the TVO using Taylor series remainders.

==> tvo_reparam.tex <==
% !TEX root = main.tex
\section{TVO Integrand Gradient Estimators}\label{app:tvo_integrand_gradients}
\subsection{Partial Derivative $\frac{\partial }{\partial \phi}$}
Recall that the TVO integral over $\beta$ includes terms of the form:
\begin{align}
\nabla_{\beta} \log Z_{\beta} = \mathbb{E}_{\pibeta} \logiw = \frac{1}{Z_{\beta}} \int \qzx^{1-\beta} \pxz^{\beta} \logiw d\vz \label{eq:tvo_integrand}
\end{align}
We proceed to differentiate this quantity in modular fashion.  In contrast to \citet{masrani2019thermodynamic}, we will use the reparameterization trick when possible.%, with the goal of improving the inference network gradient signal to noise ratio as in \cite{tucker2018doubly}.  
Concretely, reparameterization allows us to trade REINFORCE-type gradients for lower variance gradients as follows:

\begin{align}
\mathbb{E}_{\qzx} [ f(\vz) \cdot \frac{\partial}{\partial \phi} \log \qzx ] &= \mathbb{E}_{\, \epsilon \,} [ \frac{\partial }{\partial \vz} f(\vz)  \frac{\partial \vz}{\partial \phi} ]
\label{eq:reparam_general}
\end{align}

where $\vz_{i} =  g_{\phi}(\epsilon_{i})$.

We will eventually show that the partial derivative of the TVO integrand with respect to $\phi$ can be written as:
\begin{align}
\frac{\partial}{\partial \phi} \nabla_{\beta} \log Z_{\beta} &= (1- 2\beta) \mathbb{E}_{\pi_{\beta}} \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} + \beta (1-\beta) \text{Cov}_{\pi_{\beta}} \big[  \log \frac{\pxz}{\qzx}, \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} \big] \label{eq:final_tvo_integrand_cov}
\end{align}


\subsubsection{Derivation of $\frac{\partial}{\partial \phi} \nabla_{\beta} Z_{\beta} $}
Let us begin by considering $\nabla_{\beta} Z_{\beta}$.  Since we know $\nabla_{\beta} \log Z_{\beta} = \frac{1}{Z_{\beta}} \nabla_{\beta} Z_{\beta}$, we can see that this amounts to an unnormalized version of the TVO integrand \eqref{eq:tvo_integrand}.  Note that we will repeatedly use identities of the form $\frac{\partial }{\partial x} x^{\beta} = x^{\beta} \frac{\partial \log x^{\beta} }{\partial x} = \beta x^{\beta} \frac{\partial \log x}{\partial x}$.

\begin{align}
\textbf{Lemma 1:  } \frac{\partial}{\partial \phi} \nabla_{\beta} Z_{\beta} = \beta (1-\beta) \, \mathbb{E}_{\epsilon} \bigg[ w^{\beta} \, \log w   \frac{\partial  }{\partial \vz} \log w  \frac{\partial \vz}{\partial \phi} \bigg] + \textcolor{blue}{(1- 2\beta)} \, \mathbb{E}_{\, \epsilon \,}  \bigg[ w^{\beta} \, \frac{\partial }{\partial \vz} \log w  \frac{\partial \vz}{\partial \phi} \bigg] \label{eq:zb_dphi}
\end{align}

\begin{align}
\textbf{Proof: } \frac{\partial}{\partial \phi} \nabla_{\beta} Z_{\beta} &= \frac{\partial}{\partial \phi} \int \qzx^{1-\beta} \pxz^{\beta} \logiw d\vz \label{eq:def_zb_grad}\\
&= \int  \textcolor{blue}{\big(\frac{\partial }{\partial \phi} \qzx^{1-\beta} \big)} \pxz^{\beta} \logiww d\vz + \int  \qzx^{1-\beta} \pxz^{\beta} \textcolor{blue}{\frac{\partial }{\partial \phi}  \logiww} d\vz \nonumber \\
&= \int \textcolor{blue}{(1-\beta) \qzx^{-\beta} \frac{\partial \qzx}{\partial \phi}} \pxz^{\beta} \logiww d\vz + \int  \qzx^{1-\beta} \pxz^{\beta} \frac{\partial }{\partial \phi}  \logiww d\vz \nonumber \\
&= \int \textcolor{blue}{(1-\beta) \qzx^{1-\beta} \frac{\partial \log \qzx}{\partial \phi}} \pxz^{\beta} \logiww d\vz + \int \qzx^{1-\beta} \pxz^{\beta} \textcolor{blue}{\frac{\partial}{\partial \phi} [-\log \qzx]} d\vz \nonumber \\
&= \textcolor{blue}{\mathbb{E}_{\qzx} }\bigg[ \frac{\pxz^{\beta}}{\qzx^{\beta}} \big[ (1-\beta) \logiw - 1 \big] \frac{\partial \log \qzx}{\partial \phi} \bigg] \nonumber \\[1.5ex]
&= \textcolor{blue}{\mathbb{E}_{\epsilon} \frac{\partial }{\partial \vz}} \bigg[ w^{\beta} \big( (1-\beta) \logiww - 1 \big) \bigg] \textcolor{blue}{\frac{\partial \vz}{\partial \phi}} \quad \quad \text{\small (Reparameterization Trick)} \label{eq:reparam_zb} \\[1.5ex]
&= \textcolor{blue}{\beta}  \, \mathbb{E}_{\epsilon} \bigg[ \textcolor{blue}{w^{\beta-1}} \cdot \big((1-\beta) \logiww - 1 \big)  \textcolor{blue}{\frac{\partial w}{\partial \vz}}\frac{\partial \vz}{\partial \phi} \bigg] +  \, \mathbb{E}_{\epsilon} \bigg[ w^{\beta} \textcolor{blue}{\frac{\partial }{\partial \vz} (1- \beta) \logiww - 1} \frac{\partial \vz}{\partial \phi} \bigg] \nonumber \\[1.5ex] \\
&= \beta  \, \mathbb{E}_{\epsilon} \bigg[ \textcolor{blue}{w^{\beta}} \cdot \big((1-\beta) \logiww - 1 \big)  \textcolor{blue}{\frac{\partial }{\partial \vz} \logiww} \frac{\partial \vz}{\partial \phi} \bigg] + (1-\beta) \,
\mathbb{E}_{\epsilon} \bigg[ w^{\beta} \frac{\partial }{\partial \vz} \logiww \frac{\partial \vz}{\partial \phi} \bigg] \nonumber \\[1.5ex]
&= \beta (1-\beta) \, \mathbb{E}_{\epsilon} \bigg[ w^{\beta} \, \logiww  \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} \bigg] + \textcolor{blue}{(1- 2\beta)} \, \mathbb{E}_{\epsilon}  \bigg[ w^{\beta} \, \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} \bigg]
\end{align}

which we have expanded using $w = \logiw$ in the statement of the Lemma 1 above.

We will utilize this result \eqref{eq:zb_dphi} differentiating the overall TVO integrand $\nabla_{\beta} \log Z_{\beta} = \frac{1}{Z_{\beta}} \nabla_{\beta} Z_{\beta}$:
\begin{align}
\frac{\partial}{\partial \phi} \nabla_{\beta} \log Z_{\beta} &= \frac{\partial}{\partial \phi} \big( \frac{1}{Z_{\beta}} \nabla_{\beta} Z_{\beta} \big) \\
&= \big(\frac{\partial}{\partial \phi} Z_{\beta}^{-1} \big) \cdot \nabla_{\beta} Z_{\beta} + \frac{1}{Z_{\beta}} \cdot \underbrace{\frac{\partial}{\partial \phi} \nabla_{\beta} Z_{\beta}}_{Eq. \eqref{eq:zb_dphi}} \label{eq:tvo_partial_last}
\end{align}
 where Lemma 1 \eqref{eq:zb_dphi} applies to the second term.  Note that division by $Z_{\beta}$ will analytically turn $\mathbb{E}_{\epsilon} w^{\beta} [\cdot]$ terms into $\mathbb{E}_{\pibeta}[\cdot]$, as in \citet{masrani2019thermodynamic}. 


\subsubsection{Derivation  $\frac{\partial}{\partial \phi} \nabla_{\beta} \log Z_{\beta}$}\label{app:normalized_partial}
We are ultimately interested in differentiating the overall TVO integrand $\nabla_{\beta} \log Z_{\beta} = \frac{1}{Z_{\beta}} \nabla_{\beta} Z_{\beta}$ with respect to the parameters $\phi$:
\begin{align}
\frac{\partial}{\partial \phi} \nabla_{\beta} \log Z_{\beta} &= \frac{\partial}{\partial \phi} \big( \frac{1}{Z_{\beta}} \nabla_{\beta} Z_{\beta} \big) \\
&= \big(\frac{\partial}{\partial \phi} Z_{\beta}^{-1} \big) \cdot \nabla_{\beta} Z_{\beta} + \frac{1}{Z_{\beta}} \cdot \underbrace{\frac{\partial}{\partial \phi} \nabla_{\beta} Z_{\beta}}_{Eq. \eqref{eq:zb_dphi}} \label{eq:tvo_partial_last}
\end{align}
 Differentiating the first term, we will use $\tilde{\pi}_{\beta}(\vz|\vx) = \qzx^{1-\beta} \pxz^{\beta}$ to denote the unnormalized geometric mixture.
\begin{align*}
\big( \frac{\partial}{\partial \phi} Z_{\beta}^{-1} \big)  \cdot \nabla_{\beta} Z_{\beta} &= \big(\frac{\partial}{\partial \phi} Z_{\beta}^{-1} \big) \int \qzx^{1-\beta} \pxz^{\beta} \logiw d\vz \\
&= \textcolor{blue}{-\frac{1}{Z_{\beta}^2} \big( \frac{\partial}{\partial \phi} Z_{\beta} \big)} \cdot \int \textcolor{blue}{\tilde{\pi}_{\beta}} \logiw d\vz \\
&= -\frac{1}{Z_{\beta}} \textcolor{blue}{\int \big( \tilde{\pi}_{\beta} \frac{\partial}{\partial \phi} \log \tilde{\pi}_{\beta}} d\vz  \big) \cdot \textcolor{blue}{\mathbb{E}_{\pibeta} \logiw d\vz} \\
&=  - \mathbb{E}_{\pibeta} \bigg[ \frac{\partial}{\partial \phi} \log \tilde{\pi}_{\beta}(\vz|\vx) \bigg] \cdot \mathbb{E}_{\pibeta} \bigg[ \logiw \bigg]
\end{align*}
  Note that this expression appears in the covariance gradient estimator of \citet{masrani2019thermodynamic} (App. E, Eq. 51 and 61). 


However, the $\frac{\partial}{\partial \phi} \log \tilde{\pi}_{\beta}(\vz|\vx)$ term above can instead be written using the reparameterization trick as in Eq. \eqref{eq:reparam_general}:

\begin{align}
\big( \frac{\partial}{\partial \phi} Z_{\beta}^{-1} \big)  \cdot \nabla_{\beta} Z_{\beta} &= -\frac{1}{Z_{\beta}^2} \big( \frac{\partial}{\partial \phi} Z_{\beta} \big) \cdot \int \tilde{\pi}_{\beta} \logiw d\vz \nonumber \\
&= -\frac{1}{Z_{\beta}} \big( \int \tilde{\pi}_{\beta} \frac{\partial}{\partial \phi} \log \tilde{\pi}_{\beta} d\vz \big) \cdot \mathbb{E}_{\pibeta} [\logiw] d\vz \nonumber \\
&= -\frac{1}{Z_{\beta}} \textcolor{blue}{\mathbb{E}_{q_{\phi}} [\frac{\pxz^{\beta}}{\qzx^{\beta}}  \frac{\partial}{\partial \phi} (1-\beta) \log \qzx ]} \cdot \mathbb{E}_{\pi_{\beta}} [\textcolor{blue}{\log w} ] \nonumber \\
&= -\textcolor{blue}{(1-\beta)} \frac{1}{Z_{\beta}} \textcolor{blue}{\mathbb{E}_{\epsilon}} [ \textcolor{blue}{\frac{\partial }{\partial \vz} \frac{\pxz^{\beta}}{\qzx^{\beta}}} \frac{\partial \vz}{\partial \phi} ] \cdot \mathbb{E}_{\pi_{\beta}} [\log w] \nonumber  \\
&=  - (1-\beta) \mathbb{E}_{\pi_{\beta}} [\log w ] \cdot  \frac{1}{Z_{\beta}} \mathbb{E}_{\epsilon} [ \textcolor{blue}{\frac{\pxz^{\beta}}{\qzx^{\beta}} \frac{\partial }{\partial \vz} \log \frac{\pxz^{\beta}}{\qzx^{\beta}}} \frac{\partial \vz}{\partial \phi} ] \label{eq:separate_zb}\\
&=  - \textcolor{blue}{\beta} (1-\beta)  \mathbb{E}_{\pi_{\beta}} [\log \frac{\pxz}{\qzx} ] \cdot \textcolor{blue}{\mathbb{E}_{\pi_{\beta}} [ \frac{\partial }{\partial \vz} \log \frac{\pxz}{\qzx}} \frac{\partial \vz}{\partial \phi} ] \label{eq:inv_final}
\end{align}

Finally, we can combine Eq. \eqref{eq:inv_final} and Eq. \eqref{eq:zb_dphi} into Eq. \eqref{eq:tvo_partial_last}.

\begin{align}
\frac{\partial}{\partial \phi} \nabla_{\beta} \log Z_{\beta} &= \underbrace{\big(\frac{\partial}{\partial \phi} Z_{\beta}^{-1} \big) \cdot \nabla_{\beta} Z_{\beta}}_{Eq. \eqref{eq:inv_final}} + \frac{1}{Z_{\beta}} \cdot \underbrace{\frac{\partial}{\partial \phi} \nabla_{\beta} Z_{\beta}}_{Eq. \eqref{eq:zb_dphi}} \nonumber \\[1.5ex]
&= - \beta (1-\beta) [ \mathbb{E}_{\pi_{\beta}} \log \frac{\pxz}{\qzx} ][ \mathbb{E}_{\pi_{\beta}}  \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} ] + \beta (1-\beta) \mathbb{E}_{\pi_{\beta}}  [ \log \frac{\pxz}{\qzx}\frac{\partial \log w}{\partial \vz}  \frac{\partial \vz}{\partial \phi}] \nonumber \\
&\phantom{=====} + (1- 2\beta) \mathbb{E}_{\pi_{\beta}} \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} \label{eq:final_tvo_integrand2}\\
&= (1- 2\beta) \mathbb{E}_{\pi_{\beta}} \big[ \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} \big] + \beta (1-\beta) \text{Cov}_{\pi_{\beta}} \big[  \log \frac{\pxz}{\qzx}, \frac{\partial \log w }{\partial \vz} \frac{\partial \vz}{\partial \phi} \big] \label{eq:final_tvo_integrand_cov2}
\end{align}

Recall that  \citet{masrani2019thermodynamic}  obtain a similar gradient estimator, consisting of an expected gradient $\frac{\partial }{\partial \phi} \log w$ and a covariance term involving $\frac{\partial }{\partial \phi} \log \tilde{\pi}_{\beta}(\vz|\vx)$.  However, due to our use of the reparameterization trick, we instead take a `path derivative' $\frac{\partial }{\partial \vz} \log w  \frac{\partial \vz}{\partial \phi}$ and obtain scaling factors involving $\beta$.  We also note that the $\log w$  and $\log \tilde{\pi}_{\beta}(\vz|\vx)$ terms appearing in the covariance terms of Eq. \eqref{eq:final_tvo_integrand_cov2} and \citet{masrani2019thermodynamic}, respectively, differ by a factor of $\log \qzx$.






